Understanding accountability in algorithmic supply chains

Academic and policy proposals on algorithmic accountability often seek to understand algorithmic systems in their socio-technical context, recognising that they are produced by 'many hands'. Increasingly, however, algorithmic systems are also produced, deployed, and used within a supply chain comprising multiple actors tied together by flows of data between them. In such cases, it is the working together of an algorithmic supply chain of different actors who contribute to the production, deployment, use, and functionality that drives systems and produces particular outcomes. We argue that algorithmic accountability discussions must consider supply chains and the difficult implications they raise for the governance and accountability of algorithmic systems. In doing so, we explore algorithmic supply chains, locating them in their broader technical and political economic context and identifying some key features that should be understood in future work on algorithmic governance and accountability (particularly regarding general purpose AI services). To highlight ways forward and areas warranting attention, we further discuss some implications raised by supply chains: challenges for allocating accountability stemming from distributed responsibility for systems between actors, limited visibility due to the accountability horizon, service models of use and liability, and cross-border supply chains and regulatory arbitrage

==> s4.old.tex <==
\section{(Implications for) Accountability in algorithmic supply chains}
\label{sec:supplychainaccountability}



Algorithmic supply chains bring difficult implications for governance and accountability. Much algorithmic accountability research often reflects an organisation-focused, `many hands' understanding of accountability (\S\ref{sec:algosystemaccountability}). Yet the production, deployment, and use of AI technologies in supply chains is split between multiple interdependent actors who together produce its workings and effects and whose part in producing functionality cannot be understood separately from the chain (\S\ref{sec:interdependence}). Organisation-focused framings cannot properly capture this distribution of responsibilities between actors across the stages of the AI lifecycle, which also challenges assignments of accountability in relevant legal frameworks (\S\ref{sec:distributedresponsibility}). Moreover, problems with systems can propagate widely downstream through supply chains (\S\ref{sec:propagation}), yet particular actors are often unaware of the broader chain, and the distribution of responsibilities between them make interventions like risk assessments difficult (\S\ref{sec:accountabilityhorizon}). %
It is therefore crucial for governance and accountability mechanisms to understand the actors in supply chains, what they do for each other, which of them take core roles, and the interconnections and interdependencies between them. At the same time, however, the dynamic, transient nature of supply chains (\S\ref{sec:process})---which can potentially be instantiated each time and unfold differently as data is processed---is also challenging.

Moreover, algorithmic supply chains are structured through the interaction between technological, legal, social, and political economic factors  (\S\ref{sec:structuringinterdependence}). It is therefore not enough to attend only to ways of making the technology more transparent or understandable (though this can help understand specific points in particular systems' lifecycle). Instead, algorithmic accountability work must pay attention to these broader factors: for instance, how providers leverage technology and law to structure interdependencies, integrate their operations (\S\ref{sec:integration}), consolidate their position (\S\ref{sec:consolidation}), increase their control and power while minimising legal accountability (\S\ref{sec:servitisation}), and extend their supply chains across borders to minimise cost and legal risk and maximise commercial benefit ({\S\ref{sec:arbitrage}}). The dynamics of supply chains, the legal and political economic factors influencing their structure, and the relations and interdependencies between actors that result are all significant considerations from a view of accountability \textit{as a mechanism}---one, in particular, for investigating, understanding, assessing, challenging, and contesting power. They are also important in considering who should be accountable, to whom, for what, and through which mechanisms and institutional arrangements %

\subsection{Splitting production from deployment and use makes problem framing difficult}
\label{sec:problemframing}


Many algorithmic issues stem from choices around problem definition and framing that inform system design. Complex concepts may be formalised poorly, tasks may be incompletely captured, and different contexts may be insufficiently considered \cite{selbstFairnessAbstractionSociotechnical2019}. The `many hands' problem made critical questions of identifying who framed the problem and when it was framed difficult to answer \cite{passiProblemFormulationFairness2019}. Supply chain dynamics complicate this further. The actors responsible for production have limited capacity to understand the contexts of deployment and use by others, while the actors closest to the problem---those deploying or using the system---are generally unable to influence its design. Moreover, due to the split between production and deployment, application developers necessarily engage in their own problem framing -- determining whether they need an AI service to address a particular problem and, if so, which is most suitable. Yet they may lack capacity to determine which service (if any) is most appropriate to their needs (particularly if organisations swap organisational and IT know-how for license managers~\cite{balaynDebiasingRegulatingAI2021}). This is further complicated by the fact that not all services are fungible, or adaptable to a range of different framings. Services may only accept certain kinds of input data, produce certain kinds of output data, or be amenable to certain kinds of alteration and customisation. They may be developed with particular underlying assumptions which can (or should) preclude their deployment or use in other contexts~\cite{lewicki2023aiaasfairness}. Supply chain integration may further reduce flexibility in problem framing, as technical hurdles to limit interoperability and cost implications make components less readily swappable (particularly where services are strategically bundled by providers).


More cynically, actors may encourage problem framing which increases demand for their own products and services. For example, organisations selling technologies for input data, such as cameras and other environmental sensors, may also sell workplace monitoring tools which take advantage of the data produced by these sensors. Application developers with low problem framing capacity might adopt these tools without properly identifying whether they need workplace monitoring at all. The dependency of application developers on supply chains may therefore risk the autonomy of those organisations~\cite{balaynDebiasingRegulatingAI2021}. Indeed, using 
AI services leaves healthcare, education and other established sectors vulnerable to unbundling and rebundling of their  fundamental operations, leaving each stage amenable to value extraction through servitisation~\cite{balaynDebiasingRegulatingAI2021}. %

\subsection{Responsibility for algorithmic systems is distributed between several actors}
\label{sec:distributedresponsibility}


Governance and accountability mechanisms around algorithmic systems should address the \textit{distributed responsibility} in algorithmic supply chains. Different actors control aspects of commissioning, designing, developing, deploying, using, or monitoring a particular AI technology.  %
Responsibility for the workings and outcomes of supply chains is thus distributed among several actors who may not be straightforward to identify nor consistent across instances. Even when some actors are influential, there is therefore typically no one actor in overall control of a supply chain. Existing accountability literature, however, typically assumes that (while models or input data might change) the actors and components are not an important source of instability. %
Yet directing governance and accountability mechanisms at, or allocating accountability to, the wrong actors in supply chains risks undermining the stated goals of these mechanisms. %

\subsubsection{Legal accountability and distributed responsibility. \,}

Some legal frameworks have sought to address distributed responsibility in data-driven supply chains more generally. The Court of Justice of the European Union (CJEU) has attempted to contend with this in data protection law, for example. A key question in data protection law is who is a \textit{data controller} -- in \textit{de facto} control of, and therefore primarily responsible in law for, personal data processing~\cite{EU-GDPR}. The CJEU has repeatedly held that multiple parties can be  controllers for some or all aspects of a chain of processing~\cite{mahieu2019,cobbe2021artificial,jehovan,fashionid,wirtschaftsakademie}. Where several actors have common interests in the same processing, they may be \textit{joint controllers}~\cite{EU-GDPR}; where their interests in the processing diverge, they may be \textit{separate controllers}. In doing so, the Court made several useful observations: actors can be controllers if they have influence despite not having actual access to the personal data~\cite{wirtschaftsakademie,jehovan,fashionid}, controllers are not typically responsibility for parts of the chain that precede or are subsequent to those they actually control \cite{fashionid}; controllers are responsible for data protection law within the framework of their `responsibilities, powers and capabilities'~\cite{googlespain,gcandothers}; and using another actor’s platform does not exempt a controller from their obligations~\cite{wirtschaftsakademie}. 


Recognising the plurality of actors in chains of processing is welcome, but even data protection law's more nuanced assignment of roles and responsibilities may not readily map to algorithmic supply chains~\cite{gurses2017,cobbe2021artificial,mahieu2019}. Under current understandings, AI service customers are likely data controllers (the dominant party, ultimately responsible for compliance and accountability), while providers may be \textit{data processors} (the subordinate party, acting only under the instruction of a controller, with limited obligations)~\cite{millard2021,cobbe2021artificial,mahieu2019}. Yet this assignment of legal roles and responsibilities does not describe the real interdependencies and power relations between AI service providers (who are in control of their technologies, often core actors in supply chains, potentially systemically important more generally, typically presenting customers with `take-it-or-leave-it' contracts, and to a large extent determining AI-driven functionality in customers’ applications %
through their production processes) and their customers (potentially small companies without AI expertise, typically with no access to the provider’s systems, control over them, or knowledge of how they work)~\cite{cobbe2021artificial}. Even  where providers \textit{are} likely controllers for aspects of the service---such as where they use customer data for service improvement---they typically attempt to minimise responsibility by claiming in their service agreements to be processors \cite{cobbe2021artificial}. Yet the CJEU has consistently held that the factual situation outweighs contractual or other arrangements, and regulators have contradicted claimed assignments of legal roles in other kinds of data-driven supply chains~\cite{vealeImpossibleAsksCan2022}. Challenging providers' claims, however, would involve litigation or regulatory investigation. Moreover, given the need for joint controllers to agree the division of controllers' duties and responsibilities between themselves~\cite{EU-GDPR}, it is not clear how joint controllership can work where actors don't necessarily know of each other or have any direct relationship. 

The EU’s proposed AI Act suffers from related tensions. It recognises that the ‘user’ \notejs{Should we more clearly disambiguate this for the reader, by describing how this term relates to our use of 'customer' int this paper} of an AI system may differ from its ‘provider’, and envisages circumstances where a user of an AI service does so for a purpose not intended by the provider, and thus in law becomes responsible for it~\cite{EU-AIAct}. However, this does not reflect supply chain interdependencies and dynamics, where production, deployment, and use are distributed between actors. Instead, in this circumstance, the Act would potentially make actors several steps downstream from production responsible for ensuring that the AI technology complies with production-related legal requirements around training and testing, accountability, and risk management. While the user \notejs{see above comment} would inevitably be unable to comply, the actor who developed and controls that technology and is thus factually responsible for production would face no obligations. This may incentivise actors who can never provide assurance of compliance to pretend they can -- easily done due to the Act's self-regulatory framework and limited planned regulatory capacity~\cite{vealeDemystifyingDraftEU2021}. Regulatory systems which hold supply chain actors downstream of production to account for design and development may do little to regulate those who are factually responsible for production and who benefit financially from potentially unlawful API queries, effectively shielding them from liability.

\subsubsection{Allocating accountability. \,}

Governance and accountability mechanisms should therefore be grounded more clearly in and emphasise an understanding of the distribution of responsibility in algorithmic supply chains. Not \textit{every} actor in a supply chain will be responsible for the outcome of the algorithmic system -- some will provide only supporting services which do not meaningfully affect outcomes. Neither will actors who \textit{are} in some way responsible be \textit{equally} responsible -- some play a bigger role than others in determining outcomes. Nor will they be responsible for the \textit{whole} supply chain -- different actors control different aspects of it. Accountability should thus be allocated to actors across supply chains based on a proper understanding of their technological and political economic dynamics. This requires processes and criteria for identifying the distribution of responsibility across supply chains and allocating accountability to those actors, for which activities, accounting to whom, and with what possible consequences. 

It will therefore be important to understand the distribution of responsibility in algorithmic supply chains in terms of who is doing what for whom, who is performing what key functions for others, who is core to certain supply chains, and who is systemically important. Particular attention is needed due to systemically important actors -- at the time of writing, primarily Amazon, Google, Microsoft, and perhaps a few others. Though technological and political economic dynamics tend towards consolidation around these companies, and though non-AI services often provide supporting infrastructure, it will still be important to have ways to determine which aspects of supply chains are key to their outcomes and effects, as opposed to those which  could be interchanged without affecting those things. The latter, while potentially significant in their own right, are perhaps less of an urgent subject of governance and accountability mechanisms than the former.

\subsection{The \textit{accountability horizon} limits visibility and makes risk management difficult}
\label{sec:accountabilityhorizon}






Many academic, policy, and legislative initiatives in recent years have proposed impact assessments, risk assessments, and risk management mechanisms to mitigate harms caused by or with AI technologies (for example, ~\cite{EU-AIAct,cobbe2021reviewable,javadi2020monitoring,edwards2017slave,koene2019,krollaa,hutchinson2021towards,raji2020closing,williams2021,kaminski2021,rader2018explanations,ico2020,arrieta2020,canadaAlgAssess,ainow,lee2021risk,krafft2021action,saleiro2018aequitas,mitchell2019model,gebru2018datasheets,metaxa2021auditing,demos2020,adalovelace2020}). These governance and accountability mechanisms require knowledge of both the AI technology's specification and development (i.e. production) \textit{and} the purpose and context of its application (deployment). Yet the \textbf{accountability horizon} in algorithmic supply chains---the point beyond which an actor cannot ‘see’, which depends on the actor and the supply chain---challenges such mechanisms. Supply chain actors will generally be able to know whom they interact with directly (a first ‘step’ in the chain), and perhaps whom those first step actors interact with in turn (a second ‘step’), but may not understand (or be able to find out about) the data flows and interconnections beyond~\cite{cobbe2019whatlies,singh2019decprov}. Moreover, distributing responsibility for production and deployment between actors (\S\ref{sec:distributedresponsibility}) means  each has incomplete information even if they \textit{do} know who is up- and downstream of them. AI service providers, in control of production, may therefore lack knowledge of downstream contexts and use-cases of application deployments~\cite{lewicki2023aiaasfairness}. Those responsible for deployment and use typically lack access to models and often to information about their specification, training, testing, validation, and so on (and thus may have limited understanding of their capabilities and limitations). Even where they have some knowledge, models are regularly updated, and they may lack visibility, capacity, or both, to reassess. In many cases, therefore, no actor will have sufficient knowledge of or control over both production and deployment to be able to reliably assess or mitigate the impacts and risks. 

The accountability horizon thus poses major problems for accountability. Yet organisation-focused tools to provide information on points in the AI lifecycle (such as ~\cite{gebru2018datasheets,mitchell2019model}) are of limited help where information on  interconnections between actors is needed. A particular difficulty is that accountability is contextual~\cite{cobbe2021reviewable,williams2021,wieringa2020account,bovens2006,AnannyCrawford_2018}. The information needed to account for an algorithmic system depends on the actors responsible for its development, deployment, and use, on the forum owed the account, and on the broader context~\cite{cobbe2021reviewable}. As such, mechanisms to record, process, and provide information about algorithmic systems---such as ~\cite{gebru2018datasheets,mitchell2019model,arnold2019factsheets,kroll2021traceability,cloete2021droiditor,crisan2022interactivemc}---are 
also contextual. %
Yet the accountability horizon  makes understanding context difficult for actors who account for their part in algorithmic supply chains. They may not know whom they need to account to, so may not know what information to retain, about what aspects of their processes, and in what form.
They may also not know which actors upstream from them they can obtain accounts from. 



Various interventions may help expand the accountability horizon and better place actors to (i) know more about their own supply chains, and (ii) support others in knowing more about theirs. Tracking data flow between actors could help understand interconnections beyond the first few steps~\cite{singh2019decprov}, as could legal and institutional mechanisms requiring information about arrangements. ‘Know your customer’ requirements around customer on-boarding for AI services (common in financial services) could help providers understand customers’ purposes and intentions~\cite{cobbe2021artificial} (though these may only give some visibility over one or two steps in the chain). Moreover, recent CJEU data protection jurisprudence regarding transparency rights confirms that data subjects have the right to know the identity of any recipients of their personal data~\cite{osterreichische}, which may help them understand data flows. However, where the recipients' identity is not known to the data controller---which may be common due to the accountability horizon---data subjects can instead be told about the \textit{categories} of recipients of the data~\cite{osterreichische} (significantly less useful information). %
\todo{note the aside - any visibility/info provided must be relevant to actor~\cite{norval2022disclosures,cobbe2021reviewable} as is important for revealing info about supp chains, but challenging when don't know who's potentially upstream/downstream, their capabilities, what they need to know , etc }
In general, the difficulties of risk management with a split between production and deployment are not easily overcome. It is not clear, therefore, whether risk management approaches to governance and accountability of AI technologies are appropriate in this context (despite their importance in emerging laws applying to algorithmic systems, such as the EU’s AI Act~\cite{EU-AIAct}).


\subsection{Servitised distribution models give providers control beyond deployment while minimising liability}
\label{sec:servitisation}



Nissenbaum argued that the trend in the mid-1990s was for software vendors to demand property protection for their products while denying, as far as possible, accountability for them~\cite{nissenbaum1996}. Software would come with agreements which precluded \textit{ownership} by the user (instead licensed to use a copy) and emphasised the producer’s rights, while disclaiming their legal accountability for the software or anything it might do -- even where harms resulted directly from defects in it~\cite{nissenbaum1996} (though such attempts to shift liability may be invalid %
in some jurisdictions
~\cite{michelsStandardContractsCloud2021,reedConsumerProtectionCloud2021}). %
This can be understood as developers attempting to maintain control over their software to the extent possible given the distribution model at the time (typically physical media), generating artificial scarcity for an information product to maximise revenue, with minimal risk and responsibility. This produces, as Nissenbaum puts it, a ‘vacuum’ of accountability~\cite{nissenbaum1996}.

Agile turn has resulted in a change in software's distribution model, away from (licensed) physical media to the service-based, API-centric models we describe above~\cite{gurses2017}. %
Afforded in part by advances in data processing and networking technologies (\S\ref{sec:structuringinterdependence}), this \textit{servitisation} has offered providers new avenues to extend control past the point of deployment. Where vendors once sought expansive intellectual property protections, for instance, service providers today seek to maximise control over their technologies by  reserving rights to dictate terms of use and change, withdraw, or cancel products and services at will. Providers disclaim legal accountability for things that happen through use of their services~\cite{kamarinou2015,turton2021,michelsStandardContractsCloud2021}, and attempt to position themselves as data processors (\S\ref{sec:distributedresponsibility}) even where they are using customer data for their own purposes and will thus likely be the controller for that processing~\cite{cobbe2021artificial}. The asymmetrical interdependence of actors in algorithmic supply chains (\S\ref{sec:structuringinterdependence}) allows providers, who again depend less on individual customers than those customers may depend on them, to impose standard-form service agreements for most customers on a take-it-or-leave-it basis~\cite{millard2021}. Providers can thus use a combined techno-legal strategy to position themselves advantageously in markets and shape supply chains to maximise revenue and reduce risk \cite{cohenPiracySecurityArchitectures2012,cohen2019}. APIs can be used as `projections'~\cite{bucherObjectsIntenseFeeling2013} of the asymmetric balances of power between providers and customers to destabilise attempts to hold them to account: using APIs as tools to shutter businesses, destabilise research relations, and evade scrutiny~\cite{ausloosResearchingDataRights2020}, while contractually giving themselves those rights and exercising the power through changes in information policy as a form of control~\cite{reidenbergLexInformaticaFormulation1998}. 






\subsection{Cross-border supply chains permit regulatory arbitrage}
\label{sec:arbitrage}

As we describe, data processing and networking technologies afford a geographical distribution of AI production and deployment  (\S\ref{sec:structuringinterdependence}). The same technologies allow various production-related activities to themselves be distributed geographically, incentivised by jurisdictional differences in cost and regulation. This allows regulatory arbitrage, where companies in one jurisdiction exploit legal and political economic conditions in other jurisdictions to maximise commercial benefit while minimising legal accountability. This often involves contracting third-parties (such as Sama AI~\cite{samaAI}\todo{add >+1 example}) to undertake some aspects of production. For example, differences in privacy and data protection laws and labour protections can lower the cost and legal risk of dataset production activities like data collection, cleaning, and labelling~\cite{matusCertificationSystemsMachine2022,grayGhostWorkHow2019,timeOpenAI}. Environmental factors like cheap water and energy and lax planning and waste laws can influence the location of compute and storage~\cite{moscoDarkClouds2014}. While some laws---such as the EU's data protection law~\cite{EU-GDPR} and AI Act~\cite{EU-AIAct} and California's Consumer Privacy Act~\cite{US-CCPA}---have sought extra-territorial effect to address regulatory arbitrage, the cross-border nature of supply chains and difficulties of enforcement remains a significant accountability challenge.







